Sequential Latent Spaces for Modeling the Intention During Diverse Image Captioning

Diverse and accurate vision+language modeling is an important goal to retain creative freedom and maintain user engagement. However, adequately capturing the intricacies of diversity in language models is challenging. Recent works commonly resort to latent variable models augmented with more or less supervision from object detectors or part-of-speech tags. Common to all those methods is the fact that the latent variable either only initializes the sentence generation process or is identical across the steps of generation. Both methods offer no fine-grained control. To address this concern, we propose Seq-CVAE which learns a latent space for every word position. We encourage this temporal latent space to capture the 'intention' about how to complete the sentence by mimicking a representation which summarizes the future. We illustrate the efficacy of the proposed approach to anticipate the sentence continuation on the challenging MSCOCO dataset, significantly improving diversity metrics compared to baselines while performing on par w.r.t sentence quality.

==> tables/consensus.tex <==
\begin{table*}[!t]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l|c|llllllll|l|cc}
	Method & \multirow{2}{*}{\specialcell{Beam size \\ or \#samples}}  & \multicolumn{8}{c|}{Best-1 Consensus Re-ranking Accuracy} & \multirow{2}{*}{\specialcell{ Speed \\ (s/img)}} & Speed & Accuracy \\ 
	& & B4 & B3 & B2 & B1 & C &  R & M & & & & \\
\toprule
	\specialcell{Beam search \\ (w. Likelihood)} & \multirow{5}{*}{20} & 0.305 & 0.402$^\times$ & 0.538$^\times$ & 0.709$^\times$ & 0.947$^\times$ & 0.523 & 0.248 & 0.175 & 3.19 & $\times$ & $\times$ \\
	Beam search & & 0.319 & 0.423 & 0.564 & 0.733 & 1.018 & 0.537$^\checkmark$ & 0.255 & 0.185 & 7.41 & $\times$ & \checkmark \\
	Div-BS~\cite{Vijayakumar2018DiverseBS}  & & 0.320$^\checkmark$ & 0.424$^\checkmark$ & 0.562 &  0.729 &   1.032$^\checkmark$ &  0.536$^\checkmark$ &  0.255$^\checkmark$ &  0.184 &  7.60$^\times$ & $\times$ & \checkmark \\
	AG-CVAE~\cite{Wang2017DiverseAA} & & 0.299$^\times$ & 0.402$^\times$ & 0.544 & 0.716 & 0.963 & 0.518$^\times$ & 0.237$^\times$ & 0.173$^\times$ & - & - & $\times$ \\
	POS  & & 0.306 & 0.419 & 0.570$^\checkmark$ & 0.744$^\checkmark$ & 1.014 & 0.531 & 0.252 & 0.188$^\checkmark$ & 1.13$^\checkmark$ & \checkmark & \checkmark \\
% 	POS+Joint  & & 0.305 & 0.415 & 0.563 & 0.737 & 1.020 & 0.531 & 0.251 & 0.185 & 1.13$^\checkmark$ & \checkmark & \checkmark \\
    Seq-CVAE  & & - & - & - & - & - & - & - & - & - & \checkmark & \checkmark \\
    \specialcell{Seq-CVAE \\ (w. ELMO)}  & & - & - & - & - & - & - & - & - & - & \checkmark & \checkmark \\

\toprule
  
	\specialcell{Beam search \\ (w. Likelihood)} & \multirow{5}{*}{100} & 0.300$^\times$ & 0.397$^\times$ & 0.532$^\times$ & 0.703$^\times$ & 0.937$^\times$ & 0.519$^\times$ & 0.246 & 0.174$^\times$ & 18.24 & $\times$ & $\times$ \\
	Beam search  & & 0.317 & 0.419 & 0.558 & 0.729 & 1.020 & 0.532 & 0.253 & 0.186 & 40.39$^\times$ & $\times$ & \checkmark \\
	Div-BS~\cite{Vijayakumar2018DiverseBS} & & 0.325$^\checkmark$ & 0.430$^\checkmark$ & 0.569$^\checkmark$ &  0.734 & 1.034 & 0.538$^\checkmark$ &  0.255$^\checkmark$ &  0.187 &  39.71 & $\times$ & \checkmark \\
	AG-CVAE~\cite{Wang2017DiverseAA} & & 0.311 & 0.417 & 0.559 & 0.732 & 1.001 & 0.528 & 0.245$^\times$ & 0.179 & - & - & $\times$ \\
	POS & & 0.311 & 0.421 & 0.567 & 0.737 & 1.036 & 0.530 & 0.253 & 0.188$^\checkmark$ & 7.54 & \checkmark & \checkmark \\
	Seq-CVAE  & & - & - & - & - & - & - & - & - & - & \checkmark & \checkmark \\
    \specialcell{Seq-CVAE \\ (w. ELMO)}  & & - & - & - & - & - & - & - & - & - & \checkmark & \checkmark \\
\end{tabular}%
\caption{}
\vspace{-.3cm}
\label{tab:consensus}
\end{table*}


==> tables/karparthy_test.tex <==
\begin{table*}[!t]
\centering
%\setlength{\tabcolsep}{2pt}
\footnotesize
% \setlength\tabcolsep{2pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lcllllllll}
	Method & \multirow{2}{*}{\specialcell{Beam size \\ or \#samples}}  & \multicolumn{8}{c}{Best-1 Oracle Accuracy on Karparthy Test Split} \\ 
	& & B4 & B3 & B2 & B1 & C &  R & M & S \\
\toprule

	Beam search & \multirow{5}{*}{20}  & 0.543 & 0.671 & 0.787 & 0.898 & 1.707 & 0.727 & 0.427 & - \\ 
	Div-BS~\cite{Vijayakumar2018DiverseBS} & & 0.507 & 0.639 & 0.762 & 0.891 & 1.624 & 0.703 & 0.3959 & - \\
    Seq-CVAE  & & - & - & - & - & - & - & - & -\\
    \specialcell{Seq-CVAE}  & & - & - & - & - & - & - & - & - \\

\toprule
	Beam Search & \multirow{5}{*}{100}   & 0.689 & 0.782 & 0.866 & 0.945 & 1.998 & 0.798 & 0.517 & - \\
	Div-BS~\cite{Vijayakumar2018DiverseBS}  & & 0.564 & 0.671 & 0.782 & 0.904 & 1.719 & 0.727 & 0.425 &\\
	Seq-CVAE  & & - & - & - & - & - & - & - & -\\
    \specialcell{Seq-CVAE}  & & - & - & - & - & - & - & - & -\\
\end{tabular}%
\caption{}
\vspace{-.3cm}
\label{tab:karparthy_split}
\end{table*}


